Sharpness-aware Orthogonalized Momentum Algorithms

Adversarial sharpness penalty per iteration of a base optimizer, known as sharpness-aware minimization (SAM), is an accepted technique to improve generalization in deep learning. Recently, Muon has emerged as a dominant optimization algorithm for training large language models (LLMs). It achieves lower sample complexity for heavy-tailed gradient updates - a phenomenon common in LLM training. However, sharpness penalties with Muon updates are yet largely unexplored in the literature. Moreover, the behavior of SAM under heavy-tailed noise is unknown both theoretically and empirically. A potential reason for this gap is the additional cost of extra gradient computation per iteration for penalty perturbations in SAM, which becomes prohibitive for LLMs. This paper introduces Sharpness-aware Orthogonalized Momentum Algorithm (SOMA) to combine a computationally efficient and theoretically grounded perturbation scheme with the Muon algorithm. The key idea is to use stale (purely) stochastic gradient noise for adversarial perturbations. Theoretically, we show that SOMA's sample complexity is invariant to the perturbation direction. We provide explorations and insights into SOMA's robustness to heavy-tailed gradient noise. We extensively explore SOMA's efficacy in (a) mitigating quality degradation due to post-training quantization, and (b) catastrophic forgetting during fine-tuning of LLMs.

==> SOMA_exp2/common/preamble.tex <==
% AUTO-GENERATED by tools/make_tikz.py
\usepackage{pgfplots}
\usepgfplotslibrary{groupplots}
\pgfplotsset{compat=1.17}
\providecommand{\figroot}{paper_figures}  % folder that contains data/

\definecolor{c-adam}{HTML}{000000}
\pgfplotsset{os-adam/.style={color=c-adam, solid, line width=0.7pt, mark=none}}
\definecolor{c-sgd}{HTML}{7F7F7F}
\pgfplotsset{os-sgd/.style={color=c-sgd, solid, line width=0.7pt, mark=none}}
\definecolor{c-muon}{HTML}{0072B2}
\pgfplotsset{os-muon/.style={color=c-muon, solid, line width=0.7pt, mark=none}}
\definecolor{c-sam}{HTML}{E69F00}
\pgfplotsset{os-sam/.style={color=c-sam, solid, line width=0.7pt, mark=none}}
\definecolor{c-fsam}{HTML}{E69F00}
\pgfplotsset{os-fsam/.style={color=c-fsam, densely dashed, line width=0.7pt, mark=none}}
\definecolor{c-muon-sam}{HTML}{56B4E9}
\pgfplotsset{os-muon-sam/.style={color=c-muon-sam, densely dashed, line width=0.7pt, mark=none}}
\definecolor{c-fsam-ortho-muon}{HTML}{009E73}
\pgfplotsset{os-fsam-ortho-muon/.style={color=c-fsam-ortho-muon, solid, line width=0.7pt, mark=none}}
\definecolor{c-fsam-ortho-muon-stale-momentum}{HTML}{CC79A7}
\pgfplotsset{os-fsam-ortho-muon-stale-momentum/.style={color=c-fsam-ortho-muon-stale-momentum, solid, line width=0.7pt, mark=none}}
\definecolor{c-randsam-muon}{HTML}{D55E00}
\pgfplotsset{os-randsam-muon/.style={color=c-randsam-muon, densely dashed, line width=0.7pt, mark=none}}

\pgfplotsset{
  trainloss/.style={width=0.28\textwidth, height=0.24\textwidth, grid=major, grid style={gray!25}, xmin=1, xmax=64,
    tick label style={font=\tiny}, label style={font=\scriptsize}, title style={font=\scriptsize, yshift=-2pt},
    ylabel style={align=center}, scaled y ticks=false},
}


==> SOMA_exp2/train_loss_grid.tex <==
% AUTO-GENERATED by tools/make_tikz.py: rows = models, columns = datasets, lines = optimizers
\begin{tikzpicture}
\begin{groupplot}[trainloss, group style={group size=4 by 2, horizontal sep=1.0cm, vertical sep=1.5cm,
    xlabels at=edge bottom, xticklabels at=edge bottom}]
\nextgroupplot[ylabel={nanoGPT\\Fine-tuning train loss}, title={codeparrot}, legend to name=trainlosslegend, legend columns=5, legend style={font=\scriptsize, draw=none, /tikz/every even column/.append style={column sep=6pt}}]
\addplot[os-adam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/adam_codeparrot.csv};
\addlegendentry{\adamw}
% \addplot[os-sgd] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/sgd_codeparrot.csv};
% \addlegendentry{SGD}
\addplot[os-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/muon_codeparrot.csv};
\addlegendentry{\muon}
\addplot[os-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/sam_codeparrot.csv};
\addlegendentry{\sam}
\addplot[os-fsam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/fsam_codeparrot.csv};
\addlegendentry{\fsam}
\addplot[os-muon-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/muon_sam_codeparrot.csv};
\addlegendentry{\specsammuon}
\addplot[os-fsam-ortho-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/fsam_ortho_muon_codeparrot.csv};
\addlegendentry{\fpsoma}
\addplot[os-fsam-ortho-muon-stale-momentum] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/fsam_ortho_muon_stale_momentum_codeparrot.csv};
\addlegendentry{\soma}
\addplot[os-randsam-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/randsam_muon_codeparrot.csv};
\addlegendentry{\randsammuon}
\nextgroupplot[title={stackmathqa}]
\addplot[os-adam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/adam_stackmathqa.csv};
% \addplot[os-sgd] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/sgd_stackmathqa.csv};
\addplot[os-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/muon_stackmathqa.csv};
\addplot[os-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/sam_stackmathqa.csv};
\addplot[os-fsam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/fsam_stackmathqa.csv};
\addplot[os-muon-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/muon_sam_stackmathqa.csv};
\addplot[os-fsam-ortho-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/fsam_ortho_muon_stackmathqa.csv};
\addplot[os-fsam-ortho-muon-stale-momentum] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/fsam_ortho_muon_stale_momentum_stackmathqa.csv};
\addplot[os-randsam-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/randsam_muon_stackmathqa.csv};
\nextgroupplot[title={musicpile}]
\addplot[os-adam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/adam_musicpile.csv};
% \addplot[os-sgd] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/sgd_musicpile.csv};
\addplot[os-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/muon_musicpile.csv};
\addplot[os-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/sam_musicpile.csv};
\addplot[os-fsam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/fsam_musicpile.csv};
\addplot[os-muon-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/muon_sam_musicpile.csv};
\addplot[os-fsam-ortho-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/fsam_ortho_muon_musicpile.csv};
\addplot[os-fsam-ortho-muon-stale-momentum] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/fsam_ortho_muon_stale_momentum_musicpile.csv};
\addplot[os-randsam-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/randsam_muon_musicpile.csv};
\nextgroupplot[title={tulu3}]
\addplot[os-adam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/adam_tulu3.csv};
% \addplot[os-sgd] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/sgd_tulu3.csv};
\addplot[os-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/muon_tulu3.csv};
\addplot[os-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/sam_tulu3.csv};
\addplot[os-fsam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/fsam_tulu3.csv};
\addplot[os-muon-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/muon_sam_tulu3.csv};
\addplot[os-fsam-ortho-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/fsam_ortho_muon_tulu3.csv};
\addplot[os-fsam-ortho-muon-stale-momentum] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/fsam_ortho_muon_stale_momentum_tulu3.csv};
\addplot[os-randsam-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/nanogpt/randsam_muon_tulu3.csv};
\nextgroupplot[ylabel={Pythia-70M\\Fine-tuning train loss}, xlabel={Fine-tuning step}]
\addplot[os-adam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/adam_codeparrot.csv};
% \addplot[os-sgd] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/sgd_codeparrot.csv};
\addplot[os-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/muon_codeparrot.csv};
\addplot[os-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/sam_codeparrot.csv};
\addplot[os-fsam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/fsam_codeparrot.csv};
\addplot[os-muon-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/muon_sam_codeparrot.csv};
\addplot[os-fsam-ortho-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/fsam_ortho_muon_codeparrot.csv};
\addplot[os-fsam-ortho-muon-stale-momentum] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/fsam_ortho_muon_stale_momentum_codeparrot.csv};
\addplot[os-randsam-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/randsam_muon_codeparrot.csv};
\nextgroupplot[xlabel={Fine-tuning step}]
\addplot[os-adam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/adam_stackmathqa.csv};
% \addplot[os-sgd] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/sgd_stackmathqa.csv};
\addplot[os-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/muon_stackmathqa.csv};
\addplot[os-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/sam_stackmathqa.csv};
\addplot[os-fsam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/fsam_stackmathqa.csv};
\addplot[os-muon-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/muon_sam_stackmathqa.csv};
\addplot[os-fsam-ortho-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/fsam_ortho_muon_stackmathqa.csv};
\addplot[os-fsam-ortho-muon-stale-momentum] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/fsam_ortho_muon_stale_momentum_stackmathqa.csv};
\addplot[os-randsam-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/randsam_muon_stackmathqa.csv};
\nextgroupplot[xlabel={Fine-tuning step}]
\addplot[os-adam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/adam_musicpile.csv};
% \addplot[os-sgd] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/sgd_musicpile.csv};
\addplot[os-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/muon_musicpile.csv};
\addplot[os-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/sam_musicpile.csv};
\addplot[os-fsam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/fsam_musicpile.csv};
\addplot[os-muon-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/muon_sam_musicpile.csv};
\addplot[os-fsam-ortho-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/fsam_ortho_muon_musicpile.csv};
\addplot[os-fsam-ortho-muon-stale-momentum] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/fsam_ortho_muon_stale_momentum_musicpile.csv};
\addplot[os-randsam-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/randsam_muon_musicpile.csv};
\nextgroupplot[xlabel={Fine-tuning step}]
\addplot[os-adam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/adam_tulu3.csv};
% \addplot[os-sgd] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/sgd_tulu3.csv};
\addplot[os-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/muon_tulu3.csv};
\addplot[os-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/sam_tulu3.csv};
\addplot[os-fsam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/fsam_tulu3.csv};
\addplot[os-muon-sam] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/muon_sam_tulu3.csv};
\addplot[os-fsam-ortho-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/fsam_ortho_muon_tulu3.csv};
\addplot[os-fsam-ortho-muon-stale-momentum] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/fsam_ortho_muon_stale_momentum_tulu3.csv};
\addplot[os-randsam-muon] table[col sep=comma, x=step, y=train_loss]{\figroot/data/pythia70m/randsam_muon_tulu3.csv};
\end{groupplot}
\end{tikzpicture}


==> atlas_opt_cpt_curves_old/common/preamble.tex <==
% AUTO-GENERATED by tools/make_curves.py
\usepackage{pgfplots}
\usepgfplotslibrary{groupplots}
\pgfplotsset{compat=1.17}
\providecommand{\curvesroot}{atlas_opt_cpt_curves}  % folder that contains data/
\providecommand{\fitwidth}[1]{\resizebox{\ifdim\width>\textwidth\textwidth\else\width\fi}{!}{#1}}  % shrink to the text width only if wider

\definecolor{ccv-adam}{HTML}{8E0000}
\tikzset{cv-adam/.style={color=ccv-adam, solid, line width=0.9pt}}
\definecolor{ccv-sam-adam}{HTML}{D32F2F}
\tikzset{cv-sam-adam/.style={color=ccv-sam-adam, dashed, line width=0.9pt}}
\definecolor{ccv-fsam-adam}{HTML}{F06A5F}
\tikzset{cv-fsam-adam/.style={color=ccv-fsam-adam, dotted, line width=0.9pt}}
\definecolor{ccv-sgd}{HTML}{0D2A6B}
\tikzset{cv-sgd/.style={color=ccv-sgd, solid, line width=0.9pt}}
\definecolor{ccv-sam}{HTML}{1565C0}
\tikzset{cv-sam/.style={color=ccv-sam, dashed, line width=0.9pt}}
\definecolor{ccv-fsam}{HTML}{2E8BE6}
\tikzset{cv-fsam/.style={color=ccv-fsam, dotted, line width=0.9pt}}
\definecolor{ccv-msam}{HTML}{5AB0F5}
\tikzset{cv-msam/.style={color=ccv-msam, dashdotted, line width=0.9pt}}
\definecolor{ccv-muon}{HTML}{0A3D0A}
\tikzset{cv-muon/.style={color=ccv-muon, solid, line width=0.9pt}}
\definecolor{ccv-muon-sam}{HTML}{1B7A3A}
\tikzset{cv-muon-sam/.style={color=ccv-muon-sam, dashed, line width=0.9pt}}
\definecolor{ccv-fsam-ortho-muon}{HTML}{2FA05A}
\tikzset{cv-fsam-ortho-muon/.style={color=ccv-fsam-ortho-muon, dotted, line width=0.9pt}}
\definecolor{ccv-fsam-ortho-muon-stale-momentum}{HTML}{00897B}
\tikzset{cv-fsam-ortho-muon-stale-momentum/.style={color=ccv-fsam-ortho-muon-stale-momentum, dashdotted, line width=0.9pt}}
\definecolor{ccv-randsam-muon}{HTML}{5DBB63}
\tikzset{cv-randsam-muon/.style={color=ccv-randsam-muon, densely dashed, line width=0.9pt}}
\definecolor{ccv-soma-prens5}{HTML}{7CB342}
\tikzset{cv-soma-prens5/.style={color=ccv-soma-prens5, loosely dashed, line width=0.9pt}}
\definecolor{ccv-op-soma-postns5}{HTML}{A5D86E}
\tikzset{cv-op-soma-postns5/.style={color=ccv-op-soma-postns5, densely dashdotted, line width=0.9pt}}
\definecolor{ccv-msoma}{HTML}{33691E}
\tikzset{cv-msoma/.style={color=ccv-msoma, loosely dotted, line width=0.9pt}}
% legend: line sample + the paper's name macros (\muon, \soma, ... from your preamble); 2 rows x 8 aligned columns, placed above the plots
\newcommand{\legsw}[2]{\tikz[baseline=-0.55ex]\draw[#1, line width=1.2pt] (0,0)--(0.7,0);\,{\scriptsize #2}}
\newcommand{\curveslegend}{{\centering\fitwidth{\begin{tabular}{@{}l@{\hspace{1.3em}}l@{\hspace{1.3em}}l@{\hspace{1.3em}}l@{\hspace{1.3em}}l@{\hspace{1.3em}}l@{\hspace{1.3em}}l@{\hspace{1.3em}}l@{}}
  \legsw{cv-muon}{\muon} & \legsw{cv-muon-sam}{\specsammuon} & \legsw{cv-fsam-ortho-muon}{\fpsoma} & \legsw{cv-fsam-ortho-muon-stale-momentum}{\soma} & \legsw{cv-randsam-muon}{\randsammuon} & \legsw{cv-soma-prens5}{\opsomapre} & \legsw{cv-op-soma-postns5}{\opsomapost} & \legsw{cv-msoma}{\msoma} \\
  \legsw{cv-adam}{\adamw} & \legsw{cv-sam-adam}{\saw} & \legsw{cv-fsam-adam}{\fsaw} & \legsw{cv-sgd}{\sgd} & \legsw{cv-sam}{\sam} & \legsw{cv-fsam}{\fsam} & \legsw{cv-msam}{\msam} & 
\end{tabular}}\par}}

\pgfplotsset{
  curve axis/.style={width=\columnwidth, height=0.72\columnwidth, grid=major, grid style={gray!20}, xlabel={Epoch}, tick align=outside,
    tick label style={font=\scriptsize}, x tick label style={font=\tiny}, label style={font=\footnotesize}, title style={font=\footnotesize}, scaled y ticks=false},
  grid curve axis/.style={width=0.285\textwidth, height=0.215\textwidth, grid=major, grid style={gray!20}, tick align=outside,
    tick label style={font=\scriptsize}, x tick label style={font=\tiny}, label style={font=\footnotesize}, title style={font=\footnotesize, yshift=-2pt}, scaled y ticks=false},
}


==> atlas_opt_cpt_curves_old/figure_curves.tex <==
% AUTO-GENERATED
\begin{figure*}[t]
  \centering
  \curveslegend
  \vspace{4pt}

  \fitwidth{\input{\curvesroot/plots/grid_all.tex}}
  \caption{Training curves for different algorithms (mean over 3 seeds) on FineWeb-Edu dataset for NanoGPT and Pythia models and the CIFAR-10 dataset for Airbench CNN.}
  \label{fig:curves}
\end{figure*}


==> atlas_opt_v2_curves/common/preamble.tex <==
% AUTO-GENERATED by tools/make_curves.py
% \usepackage{pgfplots}
\usepgfplotslibrary{groupplots}
\pgfplotsset{compat=1.17}
\providecommand{\figroot}{atlas_opt_v2_curves}  % folder that contains data/

\definecolor{ccv-adam}{HTML}{000000}
\pgfplotsset{cv-adam/.style={color=ccv-adam, solid, line width=0.8pt, mark=none}}
\definecolor{ccv-sgd}{HTML}{7F7F7F}
\pgfplotsset{cv-sgd/.style={color=ccv-sgd, solid, line width=0.8pt, mark=none}}
\definecolor{ccv-muon}{HTML}{0072B2}
\pgfplotsset{cv-muon/.style={color=ccv-muon, solid, line width=0.8pt, mark=none}}
\definecolor{ccv-sam}{HTML}{E69F00}
\pgfplotsset{cv-sam/.style={color=ccv-sam, solid, line width=0.8pt, mark=none}}
\definecolor{ccv-fsam}{HTML}{E69F00}
\pgfplotsset{cv-fsam/.style={color=ccv-fsam, densely dashed, line width=0.8pt, mark=none}}
\definecolor{ccv-muon-sam}{HTML}{56B4E9}
\pgfplotsset{cv-muon-sam/.style={color=ccv-muon-sam, densely dashed, line width=0.8pt, mark=none}}
\definecolor{ccv-fsam-ortho-muon}{HTML}{009E73}
\pgfplotsset{cv-fsam-ortho-muon/.style={color=ccv-fsam-ortho-muon, solid, line width=0.8pt, mark=none}}
\definecolor{ccv-fsam-ortho-muon-stale-momentum}{HTML}{CC79A7}
\pgfplotsset{cv-fsam-ortho-muon-stale-momentum/.style={color=ccv-fsam-ortho-muon-stale-momentum, solid, line width=0.8pt, mark=none}}
\definecolor{ccv-randsam-muon}{HTML}{D55E00}
\pgfplotsset{cv-randsam-muon/.style={color=ccv-randsam-muon, densely dashed, line width=0.8pt, mark=none}}
\definecolor{ccv-soma-prens5}{HTML}{6A3D9A}
\pgfplotsset{cv-soma-prens5/.style={color=ccv-soma-prens5, solid, line width=0.8pt, mark=none}}
\definecolor{ccv-op-soma-postns5}{HTML}{8C564B}
\pgfplotsset{cv-op-soma-postns5/.style={color=ccv-op-soma-postns5, densely dashed, line width=0.8pt, mark=none}}

\pgfplotsset{
  curve axis/.style={width=\columnwidth, height=0.72\columnwidth, grid=major, grid style={gray!25}, xlabel={Epoch},
    tick label style={font=\scriptsize}, label style={font=\footnotesize}, title style={font=\footnotesize},
    legend style={font=\tiny, draw=none, fill=white, fill opacity=0.8, text opacity=1}, scaled y ticks=false},
  grid curve axis/.style={width=0.31\textwidth, height=0.25\textwidth, grid=major, grid style={gray!25},
    tick label style={font=\tiny}, label style={font=\scriptsize}, title style={font=\scriptsize, yshift=-2pt}, scaled y ticks=false},
}


==> atlas_opt_v2_curves/figure_curves.tex <==
% AUTO-GENERATED
\begin{figure*}[t]
  \centering
  \input{\curvesroot/plots/grid_all.tex}

  \vspace{3pt}
  \ref{curveslegend}
  \caption{Pretraining curves of the eleven optimizers (mean over 3 seeds) on nanoGPT, Pythia-70M and the CIFAR-10 CNN: training loss, validation accuracy and validation perplexity per epoch.}
  \label{fig:curves}
\end{figure*}


==> dataforsyntheticplots/nn_aniso_val_loss.tex <==
% ---- nn_aniso_val_loss
\providecolor{muonrow}{RGB}{208,236,214}\providecolor{adamrow}{RGB}{255,214,214}\providecolor{sgdrow}{RGB}{208,226,247}
\begin{table*}[t]\centering\scriptsize\setlength{\tabcolsep}{4pt}
\caption{Validation loss: best value over the perturbation radius $\rho$ and the radius $\rho^\star$ where it is attained (median of 8 seeds; Frobenius-ball methods pool the global and per-layer radius modes). Rows are grouped by base optimizer: Muon (green), AdamW (red), SGD (blue); baselines have no $\rho^\star$. Best value per $\alpha$ in bold.}\label{tab:nn_aniso_val_loss}
\begin{tabular}{lcccccccc}\toprule
Algorithm & \multicolumn{2}{c}{$\alpha=1.1$} & \multicolumn{2}{c}{$\alpha=1.6$} & \multicolumn{2}{c}{$\alpha=2.0$} & \multicolumn{2}{c}{$\alpha=3.0$} \\
& best loss & $\rho^\star$ & best loss & $\rho^\star$ & best loss & $\rho^\star$ & best loss & $\rho^\star$ \\\midrule
\rowcolor{muonrow} \muon & 2.49 & -- & 2.36 & -- & 2.51 & -- & 2.76 & -- \\
\rowcolor{muonrow} \specsammuon & 2.38 & 1 & \textbf{2.01} & 0.5 & \textbf{1.98} & 0.5 & 1.93 & 0.5 \\
\rowcolor{muonrow} \fpsoma & \textbf{2.34} & 1 & \textbf{2.01} & 0.5 & 2 & 0.5 & 1.96 & 0.5 \\
\rowcolor{muonrow} \soma & 2.39 & 1 & 2.09 & 1 & 2.05 & 1 & 2.08 & 1 \\
\rowcolor{muonrow} \randsammuon & 2.48 & 0.5 & 2.35 & 1 & 2.5 & 1 & 2.7 & 1 \\
\rowcolor{muonrow} \opsomapre & 2.4 & 1 & 2.11 & 1 & 2.06 & 1 & 2.05 & 1 \\
\rowcolor{muonrow} \opsomapost & 2.41 & 1 & 2.09 & 1 & 2.07 & 1 & 2.11 & 1 \\
\rowcolor{muonrow} \textsc{Msoma} & 2.47 & 1 & 2.36 & 0.001 & 2.52 & 0.001 & 2.74 & 0.02 \\
\rowcolor{adamrow} \adamw & 2.93 & -- & 2.08 & -- & 1.99 & -- & 1.95 & -- \\
\rowcolor{adamrow} \samadamw & 2.92 & 1 & 2.07 & 0.02 & \textbf{1.98} & 0.5 & 1.93 & 0.5 \\
\rowcolor{adamrow} \fsamadamw & 2.93 & 1 & 2.07 & 0.05 & \textbf{1.98} & 0.5 & \textbf{1.92} & 1 \\
\rowcolor{sgdrow} \sgd & 523 & -- & 55.1 & -- & 10.7 & -- & 5.04 & -- \\
\rowcolor{sgdrow} \sam & 487 & 1 & 42.5 & 1 & 7.5 & 1 & 3.83 & 1 \\
\rowcolor{sgdrow} \fsam & 494 & 1 & 42.2 & 1 & 7.34 & 1 & 3.79 & 1 \\
\rowcolor{sgdrow} \textsc{Msam} & 538 & 0.5 & 53.6 & 0.2 & 9.76 & 1 & 4.89 & 1 \\
\bottomrule\end{tabular}\end{table*}


==> dataforsyntheticplots/nn_iso_val_loss.tex <==
% ---- nn_iso_val_loss
\providecolor{muonrow}{RGB}{208,236,214}\providecolor{adamrow}{RGB}{255,214,214}\providecolor{sgdrow}{RGB}{208,226,247}
\begin{table*}[t]\centering\scriptsize\setlength{\tabcolsep}{4pt}
\caption{Validation loss: best value over the perturbation radius $\rho$ and the radius $\rho^\star$ where it is attained (median of 8 seeds; Frobenius-ball methods pool the global and per-layer radius modes). Rows are grouped by base optimizer: Muon (green), AdamW (red), SGD (blue); baselines have no $\rho^\star$. Best value per $\alpha$ in bold.}\label{tab:nn_iso_val_loss}
\begin{tabular}{lcccccccc}\toprule
Algorithm & \multicolumn{2}{c}{$\alpha=1.1$} & \multicolumn{2}{c}{$\alpha=1.6$} & \multicolumn{2}{c}{$\alpha=2.0$} & \multicolumn{2}{c}{$\alpha=3.0$} \\
& best loss & $\rho^\star$ & best loss & $\rho^\star$ & best loss & $\rho^\star$ & best loss & $\rho^\star$ \\\midrule
\rowcolor{muonrow} \muon & 2.59 & -- & 2.25 & -- & 2.37 & -- & 2.64 & -- \\
\rowcolor{muonrow} \specsammuon & 2.43 & 1 & \textbf{2.01} & 0.5 & 1.97 & 0.5 & 1.95 & 0.5 \\
\rowcolor{muonrow} \fpsoma & 2.4 & 1 & 2.02 & 0.5 & 1.97 & 0.5 & 1.95 & 0.5 \\
\rowcolor{muonrow} \soma & 2.45 & 1 & 2.08 & 1 & 2.04 & 1 & 2.04 & 1 \\
\rowcolor{muonrow} \randsammuon & 2.58 & 1 & 2.24 & 0.02 & 2.36 & 1 & 2.59 & 1 \\
\rowcolor{muonrow} \opsomapre & 2.49 & 1 & 2.09 & 1 & 2.06 & 1 & 2.04 & 1 \\
\rowcolor{muonrow} \opsomapost & 2.49 & 1 & 2.07 & 1 & 2.07 & 1 & 2.11 & 1 \\
\rowcolor{muonrow} \textsc{Msoma} & 2.58 & 1 & 2.25 & 0.02 & 2.37 & 0.01 & 2.64 & 0.002 \\
\rowcolor{adamrow} \adamw & 2.28 & -- & 2.03 & -- & 1.97 & -- & 1.94 & -- \\
\rowcolor{adamrow} \samadamw & 2.28 & 0.05 & 2.03 & 0.01 & \textbf{1.96} & 0.5 & 1.94 & 0.5 \\
\rowcolor{adamrow} \fsamadamw & \textbf{2.27} & 0.5 & 2.03 & 0.5 & \textbf{1.96} & 1 & \textbf{1.93} & 1 \\
\rowcolor{sgdrow} \sgd & 588 & -- & 57.5 & -- & 10.5 & -- & 4.94 & -- \\
\rowcolor{sgdrow} \sam & 535 & 1 & 44.8 & 1 & 6.85 & 1 & 3.76 & 1 \\
\rowcolor{sgdrow} \fsam & 538 & 1 & 44.1 & 1 & 6.72 & 1 & 3.75 & 1 \\
\rowcolor{sgdrow} \textsc{Msam} & 574 & 1 & 46 & 1 & 9.2 & 1 & 4.84 & 0.5 \\
\bottomrule\end{tabular}\end{table*}


==> dataforsyntheticplots/tables.tex <==
% ---- nn_aniso_val_acc
\begin{table*}[t]\centering\scriptsize\setlength{\tabcolsep}{4pt}
\caption{Validation accuracy (\%): best value over the perturbation radius $\rho$ and the radius $\rho^\star$ where it is attained (median of 8 seeds).}\label{tab:nn_aniso_val_acc}
\begin{tabular}{lcccccccc}\toprule
Algorithm & \multicolumn{2}{c}{$\alpha=1.1$} & \multicolumn{2}{c}{$\alpha=1.6$} & \multicolumn{2}{c}{$\alpha=2.0$} & \multicolumn{2}{c}{$\alpha=3.0$} \\
& best acc. & $\rho^\star$ & best acc.& $\rho^\star$ & best acc. & $\rho^\star$ & best acc. & $\rho^\star$ \\\midrule
\soma & 39.1 & 1.0 & 45 & 1.0 & 46.3 & 1.0 & 46.5 & 0.5 \\
\fpsoma & \textbf{39.8} & 1.0 & 44.2 & 0.5 & 46.9 & 0.5 & 46.7 & 0.5 \\
\specsammuon & 38.6 & 0.5 & 43.7 & 0.5 & 46.3 & 0.5 & 47 & 0.5 \\
\randsammuon & 38.3 & 0.01 & 43.4 & 0.5 & 44.5 & 0.1 & 44.7 & 1.0 \\
\fsam & 36.8 & 0.1 & 39.4 & 0.01 & 40.2 & 1.0 & 43 & 0.2 \\
\sam & 37.2 & 0.01 & 39.5 & 0.01 & 40.7 & 0.2 & 42.5 & 0.2 \\
\opsomapre & 38.8 & 1.0 & \textbf{45.3} & 1.0 & 46.1 & 1.0 & 46.9 & 0.5 \\
\opsomapost & 38.3 & 1.0 & 45.2 & 1.0 & \textbf{47.9} & 1.0 & \textbf{47.4} & 1.0 \\
\samadamw & 28.9 & 1.0 & 41.9 & 0.5 & 44.5 & 0.1 & 46.5 & 1.0 \\
\fsamadamw & 28.6 & 0.01 & 42 & 1.0 & 44.5 & 0.05 & 46.2 & 1.0 \\
\midrule
\muon & \multicolumn{2}{c}{38.1} & \multicolumn{2}{c}{42.9} & \multicolumn{2}{c}{44} & \multicolumn{2}{c}{44.3} \\
\adamw & \multicolumn{2}{c}{28.6} & \multicolumn{2}{c}{41.5} & \multicolumn{2}{c}{44.2} & \multicolumn{2}{c}{45.4} \\
\bottomrule\end{tabular}\end{table*}

% ---- nn_aniso_train_loss
\begin{table*}[t]\centering\scriptsize\setlength{\tabcolsep}{4pt}
\caption{Training loss: best value over the perturbation radius $\rho$ and the radius $\rho^\star$ where it is attained (median of 8 seeds).}\label{tab:nn_aniso_train_loss}
\begin{tabular}{lcccccccc}\toprule
Algorithm & \multicolumn{2}{c}{$\alpha=1.1$} & \multicolumn{2}{c}{$\alpha=1.6$} & \multicolumn{2}{c}{$\alpha=2.0$} & \multicolumn{2}{c}{$\alpha=3.0$} \\
& best loss & $\rho^\star$ & best loss& $\rho^\star$ & best loss & $\rho^\star$ & best loss & $\rho^\star$ \\\midrule
\soma & \textbf{1.43} & 0.2 & 0.371 & 0.02 & 0.184 & 0.01 & 0.0783 & 0.01 \\
\fpsoma & 1.44 & 0.2 & 0.372 & 0.01 & 0.186 & 0.02 & 0.0768 & 0.02 \\
\specsammuon & 1.45 & 0.02 & 0.375 & 0.01 & 0.187 & 0.01 & 0.0786 & 0.01 \\
\randsammuon & 1.45 & 0.1 & 0.37 & 0.5 & 0.183 & 0.2 & 0.0779 & 0.5 \\
\fsam & 8.89 & 0.5 & \textbf{0.0102} & 0.1 & 0.00729 & 0.1 & 0.0114 & 0.1 \\
\sam & 9.58 & 0.5 & 0.0117 & 0.02 & \textbf{0.00716} & 0.05 & \textbf{0.0111} & 0.2 \\
\opsomapre & 1.44 & 0.2 & 0.371 & 0.01 & 0.182 & 0.01 & 0.0779 & 0.01 \\
\opsomapost & 1.44 & 0.2 & 0.37 & 0.05 & 0.183 & 0.02 & 0.0778 & 0.05 \\
\samadamw & 2.7 & 1.0 & 1.32 & 0.01 & 1.02 & 0.01 & 0.804 & 0.01 \\
\fsamadamw & 2.7 & 0.02 & 1.32 & 0.01 & 1.02 & 0.01 & 0.804 & 0.01 \\
\midrule
\muon & \multicolumn{2}{c}{1.45} & \multicolumn{2}{c}{0.372} & \multicolumn{2}{c}{0.184} & \multicolumn{2}{c}{0.078} \\
\adamw & \multicolumn{2}{c}{2.7} & \multicolumn{2}{c}{1.32} & \multicolumn{2}{c}{1.02} & \multicolumn{2}{c}{0.803} \\
\bottomrule\end{tabular}\end{table*}

% ---- nn_aniso_val_loss
\begin{table*}[t]\centering\scriptsize\setlength{\tabcolsep}{4pt}
\caption{Validation loss: best value over the perturbation radius $\rho$ and the radius $\rho^\star$ where it is attained (median of 8 seeds).}\label{tab:nn_aniso_val_loss}
\begin{tabular}{lcccccccc}\toprule
Algorithm & \multicolumn{2}{c}{$\alpha=1.1$} & \multicolumn{2}{c}{$\alpha=1.6$} & \multicolumn{2}{c}{$\alpha=2.0$} & \multicolumn{2}{c}{$\alpha=3.0$} \\
& best loss & $\rho^\star$ & best loss& $\rho^\star$ & best loss & $\rho^\star$ & best loss & $\rho^\star$ \\\midrule
\soma & 2.39 & 1.0 & 2.09 & 1.0 & 2.05 & 1.0 & 2.08 & 1.0 \\
\fpsoma & \textbf{2.34} & 1.0 & \textbf{2.01} & 0.5 & 2 & 0.5 & 1.96 & 0.5 \\
\specsammuon & 2.38 & 1.0 & \textbf{2.01} & 0.5 & \textbf{1.98} & 0.5 & 1.93 & 0.5 \\
\randsammuon & 2.48 & 0.5 & 2.35 & 1.0 & 2.5 & 0.5 & 2.7 & 1.0 \\
\fsam & 499 & 1.0 & 46.9 & 1.0 & 8.36 & 1.0 & 4.19 & 1.0 \\
\sam & 487 & 1.0 & 45.2 & 1.0 & 8.02 & 1.0 & 4.21 & 1.0 \\
\opsomapre & 2.4 & 1.0 & 2.11 & 1.0 & 2.06 & 1.0 & 2.05 & 1.0 \\
\opsomapost & 2.41 & 1.0 & 2.09 & 1.0 & 2.07 & 1.0 & 2.11 & 1.0 \\
\samadamw & 2.92 & 1.0 & 2.08 & 0.01 & \textbf{1.98} & 0.2 & 1.93 & 1.0 \\
\fsamadamw & 2.93 & 1.0 & 2.07 & 0.1 & \textbf{1.98} & 0.5 & \textbf{1.92} & 1.0 \\
\midrule
\muon & \multicolumn{2}{c}{2.49} & \multicolumn{2}{c}{2.36} & \multicolumn{2}{c}{2.51} & \multicolumn{2}{c}{2.76} \\
\adamw & \multicolumn{2}{c}{2.93} & \multicolumn{2}{c}{2.08} & \multicolumn{2}{c}{1.99} & \multicolumn{2}{c}{1.95} \\
\bottomrule\end{tabular}\end{table*}

% ---- mse_aniso_gap
\begin{table*}[t]\centering\scriptsize\setlength{\tabcolsep}{4pt}
\caption{Optimality gap: best value over the perturbation radius $\rho$ and the radius $\rho^\star$ where it is attained (median of 8 seeds).}\label{tab:mse_aniso_gap}
\begin{tabular}{lcccccccc}\toprule
Algorithm & \multicolumn{2}{c}{$\alpha=1.1$} & \multicolumn{2}{c}{$\alpha=1.6$} & \multicolumn{2}{c}{$\alpha=2.0$} & \multicolumn{2}{c}{$\alpha=3.0$} \\
& gap & $\rho^\star$ & gap& $\rho^\star$ & gap & $\rho^\star$ & gap & $\rho^\star$ \\\midrule
\soma & 0.263 & 1.0 & 0.0551 & 0.5 & 0.0299 & 0.2 & 0.0163 & 0.1 \\
\fpsoma & \textbf{0.252} & 1.0 & \textbf{0.0457} & 0.5 & \textbf{0.0247} & 0.5 & 0.0143 & 0.2 \\
\specsammuon & 0.265 & 1.0 & 0.0473 & 0.5 & 0.0253 & 0.5 & 0.0141 & 0.5 \\
\randsammuon & 0.41 & 1.0 & 0.0612 & 1.0 & 0.0312 & 1.0 & 0.0163 & 1.0 \\
\fsam & 3.8 & 1.0 & 0.116 & 1.0 & 0.0352 & 0.2 & \textbf{0.0137} & 1.0 \\
\sam & 3.72 & 1.0 & 0.116 & 0.5 & 0.0349 & 0.01 & 0.014 & 1.0 \\
\opsomapre & 0.274 & 1.0 & 0.0548 & 0.5 & 0.0296 & 0.2 & 0.0159 & 0.2 \\
\opsomapost & 0.287 & 1.0 & 0.0537 & 0.5 & 0.0284 & 0.5 & 0.0157 & 0.2 \\
\samadamw & 0.556 & 1.0 & 0.108 & 1.0 & 0.0584 & 1.0 & 0.0362 & 0.5 \\
\fsamadamw & 0.557 & 1.0 & 0.108 & 1.0 & 0.0585 & 1.0 & 0.0361 & 1.0 \\
\midrule
\muon & \multicolumn{2}{c}{0.413} & \multicolumn{2}{c}{0.062} & \multicolumn{2}{c}{0.0316} & \multicolumn{2}{c}{0.0165} \\
\adamw & \multicolumn{2}{c}{0.559} & \multicolumn{2}{c}{0.109} & \multicolumn{2}{c}{0.0592} & \multicolumn{2}{c}{0.0364} \\
\bottomrule\end{tabular}\end{table*}

% % ---- nn_iso_val_acc
% \begin{table*}[t]\centering\scriptsize\setlength{\tabcolsep}{4pt}
% \caption{Validation accuracy (\%): best value over the perturbation radius $\rho$ and the radius $\rho^\star$ where it is attained (median of 8 seeds).}\label{tab:nn_iso_val_acc}
% \begin{tabular}{lcccccccc}\toprule
% Method & \multicolumn{2}{c}{$\alpha=1.1$} & \multicolumn{2}{c}{$\alpha=1.6$} & \multicolumn{2}{c}{$\alpha=2.0$} & \multicolumn{2}{c}{$\alpha=3.0$} \\
% & best & $\rho^\star$ & best & $\rho^\star$ & best & $\rho^\star$ & best & $\rho^\star$ \\\midrule
% SOMA & 38.2 & 1.0 & \textbf{44.8} & 1.0 & \textbf{46.6} & 0.5 & \textbf{46.6} & 0.5 \\
% FP-SOMA & 37.8 & 1.0 & 44.7 & 1.0 & \textbf{46.6} & 0.5 & 46.1 & 0.5 \\
% SpecSAM-Muon & 36.6 & 0.2 & 44.2 & 0.5 & 45.3 & 0.02 & 46.2 & 0.5 \\
% RandSAM-Muon & 36.3 & 0.05 & 43.8 & 0.1 & 45.5 & 0.5 & 44.5 & 0.2 \\
% FSAM & 36.2 & 0.5 & 41.0 & 0.5 & 39.6 & 0.2 & 42.7 & 1.0 \\
% SAM & 36.4 & 0.5 & 40.0 & 0.5 & 40.0 & 0.05 & 42.2 & 0.01 \\
% SAM-AdamW & \textbf{40.8} & 0.02 & 43.6 & 0.2 & 44.6 & 0.01 & 46.1 & 0.05 \\
% FSAM-AdamW & \textbf{40.8} & 0.02 & 43.3 & 0.1 & 44.7 & 0.05 & 46 & 0.01 \\
% \midrule
% Muon & \multicolumn{2}{c}{36.1} & \multicolumn{2}{c}{43.3} & \multicolumn{2}{c}{45.2} & \multicolumn{2}{c}{43.8} \\
% AdamW & \multicolumn{2}{c}{40.6} & \multicolumn{2}{c}{43.0} & \multicolumn{2}{c}{44.1} & \multicolumn{2}{c}{45.8} \\
% \bottomrule\end{tabular}\end{table*}

% % ---- nn_iso_train_loss
% \begin{table*}[t]\centering\scriptsize\setlength{\tabcolsep}{4pt}
% \caption{Training loss: best value over the perturbation radius $\rho$ and the radius $\rho^\star$ where it is attained (median of 8 seeds).}\label{tab:nn_iso_train_loss}
% \begin{tabular}{lcccccccc}\toprule
% Method & \multicolumn{2}{c}{$\alpha=1.1$} & \multicolumn{2}{c}{$\alpha=1.6$} & \multicolumn{2}{c}{$\alpha=2.0$} & \multicolumn{2}{c}{$\alpha=3.0$} \\
% & best & $\rho^\star$ & best & $\rho^\star$ & best & $\rho^\star$ & best & $\rho^\star$ \\\midrule
% SOMA & \textbf{1.56} & 0.5 & 0.484 & 0.02 & 0.235 & 0.02 & 0.113 & 0.01 \\
% FP-SOMA & 1.57 & 0.2 & 0.483 & 0.01 & 0.234 & 0.02 & 0.112 & 0.02 \\
% SpecSAM-Muon & 1.58 & 0.02 & 0.485 & 0.01 & 0.237 & 0.01 & 0.113 & 0.01 \\
% RandSAM-Muon & 1.58 & 0.01 & 0.482 & 0.05 & 0.233 & 0.5 & 0.113 & 0.5 \\
% FSAM & 11.8 & 0.05 & 0.0114 & 0.2 & \textbf{0.00789} & 0.1 & \textbf{0.0109} & 0.5 \\
% SAM & 11.4 & 0.2 & \textbf{0.00535} & 0.2 & 0.00828 & 0.1 & \textbf{0.0109} & 0.2 \\
% SAM-AdamW & 1.71 & 0.01 & 1.17 & 0.01 & 0.974 & 0.01 & 0.818 & 0.01 \\
% FSAM-AdamW & 1.71 & 0.01 & 1.17 & 0.01 & 0.974 & 0.01 & 0.818 & 0.01 \\
% \midrule
% Muon & \multicolumn{2}{c}{1.58} & \multicolumn{2}{c}{0.482} & \multicolumn{2}{c}{0.233} & \multicolumn{2}{c}{0.114} \\
% AdamW & \multicolumn{2}{c}{1.71} & \multicolumn{2}{c}{1.17} & \multicolumn{2}{c}{0.974} & \multicolumn{2}{c}{0.817} \\
% \bottomrule\end{tabular}\end{table*}

% % ---- nn_iso_val_loss
% \begin{table*}[t]\centering\scriptsize\setlength{\tabcolsep}{4pt}
% \caption{Validation loss: best value over the perturbation radius $\rho$ and the radius $\rho^\star$ where it is attained (median of 8 seeds).}\label{tab:nn_iso_val_loss}
% \begin{tabular}{lcccccccc}\toprule
% Method & \multicolumn{2}{c}{$\alpha=1.1$} & \multicolumn{2}{c}{$\alpha=1.6$} & \multicolumn{2}{c}{$\alpha=2.0$} & \multicolumn{2}{c}{$\alpha=3.0$} \\
% & best & $\rho^\star$ & best & $\rho^\star$ & best & $\rho^\star$ & best & $\rho^\star$ \\\midrule
% SOMA & 2.45 & 1.0 & 2.08 & 1.0 & 2.04 & 1.0 & 2.04 & 1.0 \\
% FP-SOMA & 2.4 & 1.0 & 2.02 & 0.5 & 1.97 & 0.5 & 1.95 & 0.5 \\
% SpecSAM-Muon & 2.43 & 1.0 & \textbf{2.01} & 0.5 & 1.97 & 0.5 & 1.95 & 0.5 \\
% RandSAM-Muon & 2.58 & 1.0 & 2.24 & 0.02 & 2.37 & 1.0 & 2.62 & 1.0 \\
% FSAM & 534 & 0.5 & 48.6 & 1.0 & 7.7 & 1.0 & 4.04 & 1.0 \\
% SAM & 540 & 1.0 & 48 & 1.0 & 7.81 & 1.0 & 4.07 & 1.0 \\
% SAM-AdamW & 2.28 & 0.05 & 2.03 & 0.01 & \textbf{1.96} & 0.5 & 1.94 & 1.0 \\
% FSAM-AdamW & \textbf{2.27} & 0.5 & 2.03 & 0.01 & \textbf{1.96} & 1.0 & \textbf{1.93} & 1.0 \\
% \midrule
% Muon & \multicolumn{2}{c}{2.59} & \multicolumn{2}{c}{2.25} & \multicolumn{2}{c}{2.37} & \multicolumn{2}{c}{2.64} \\
% AdamW & \multicolumn{2}{c}{2.28} & \multicolumn{2}{c}{2.03} & \multicolumn{2}{c}{1.97} & \multicolumn{2}{c}{1.94} \\
% \bottomrule\end{tabular}\end{table*}


==> paper_figures_v2/common/preamble.tex <==
% AUTO-GENERATED by tools/make_forgetting_figures.py
\usepackage{booktabs,pgfplots,pgfplotstable,xcolor}
\usepgfplotslibrary{statistics}
\pgfplotsset{compat=1.17}
\providecommand{\curveroot}{paper_figures_v2}  % folder that contains data/
\providecommand{\fitwidth}[1]{\resizebox{\ifdim\width>\textwidth\textwidth\else\width\fi}{!}{#1}}  % shrink to the text width only if wider

\definecolor{c-codeparrot}{HTML}{0072B2}
\definecolor{c-stackmathqa}{HTML}{E69F00}
\definecolor{c-musicpile}{HTML}{009E73}
\definecolor{c-tulu3}{HTML}{CC79A7}

\pgfplotsset{
  dpt bars/.style={ybar, width=\textwidth, height=0.30\textwidth, bar width=2.6pt, ymin=0, enlarge x limits=0.045,
    ymajorgrids, grid style={gray!25}, xtick=data, x tick label style={rotate=35, anchor=east, font=\scriptsize},
    tick label style={font=\scriptsize}, label style={font=\footnotesize}, title style={font=\footnotesize, yshift=0.55cm},
    xlabel={Pretraining optimizer}, ylabel={Forgetting $\Delta$PT (FineWeb loss rise)}, scaled y ticks=false,
    legend style={font=\scriptsize, at={(0.5,1.02)}, anchor=south, legend columns=5, draw=none},
    error bars/y dir=both, error bars/y explicit, error bars/error bar style={line width=0.4pt}},
}


==> paper_figures_v2/table_forgetting.tex <==
% AUTO-GENERATED: one table per model
\input{\curveroot/table_forgetting_nanogpt.tex}
\input{\curveroot/table_forgetting_pythia70m.tex}


==> paper_figures_v2/table_forgetting_nanogpt.tex <==
% AUTO-GENERATED: numbers read from data/forgetting_table_nanogpt.csv
\begin{table*}[t]
  \centering
  \small
  \caption{nanoGPT (GPT-2 small): held-out FineWeb-Edu loss $L$ of models pretrained with each optimizer, before ($L_{\text{before}}$) and after ($L_{\text{after}}$) fine-tuning on each
  of four datasets (lower is better; forgetting $\Delta\mathrm{PT}=L_{\text{after}}-L_{\text{before}}$). $L_{\text{after}}$ is taken at a common fine-tuning loss per dataset
  (target $\tau$ codeparrot: 1.690, stackmathqa: 2.291, musicpile: 3.067, tulu3: 2.215); mean $\pm$ sd over 3 seeds. ``Average'' is the mean of the four $L_{\text{after}}$ values. $\Delta\%_{\text{adj}}=100\,(L_{\text{after}}-L_{\text{before}})/(L_{\text{before}}+k)$ with
  $k=3.156$ (mean of all $L_{\text{before}}$ of this model). Bold: lowest among comparable models. $^\dagger$: $L_{\text{before}}$ clearly worse than AdamW's (perplexity $>3\%$ higher), so these rows are not comparable.}
  \label{tab:forgetting-nanogpt}
  \fitwidth{\pgfplotstabletypeset[col sep=comma, string type, every head row/.style={before row=\toprule, after row=\midrule},
    every last row/.style={after row=\bottomrule},
    columns={optimizer,before,codeparrot,stackmathqa,musicpile,tulu3,avg,smooth},
    columns/optimizer/.style={column name=Optimizer, string type, column type=l},
    columns/before/.style={column name={$L_{\text{before}}$}, string type, column type=c},
    columns/codeparrot/.style={column name={$L_{\text{after}}$ codeparrot}, string type, column type=c},
    columns/stackmathqa/.style={column name={$L_{\text{after}}$ stackmathqa}, string type, column type=c},
    columns/musicpile/.style={column name={$L_{\text{after}}$ musicpile}, string type, column type=c},
    columns/tulu3/.style={column name={$L_{\text{after}}$ tulu3}, string type, column type=c},
    columns/avg/.style={column name={$L_{\text{after}}$ average}, string type, column type=c},
    columns/smooth/.style={column name={$\Delta\%_{\text{adj}}$}, string type, column type=c}]{\curveroot/data/forgetting_table_nanogpt.csv}}
\end{table*}


==> paper_figures_v2/table_forgetting_pythia70m.tex <==
% AUTO-GENERATED: numbers read from data/forgetting_table_pythia70m.csv
\begin{table*}[t]
  \centering
  \small
  \caption{Pythia-70M: held-out FineWeb-Edu loss $L$ of models pretrained with each optimizer, before ($L_{\text{before}}$) and after ($L_{\text{after}}$) fine-tuning on each
  of four datasets (lower is better; forgetting $\Delta\mathrm{PT}=L_{\text{after}}-L_{\text{before}}$). $L_{\text{after}}$ is taken at a common fine-tuning loss per dataset
  (target $\tau$ codeparrot: 2.232, stackmathqa: 2.459, musicpile: 3.379, tulu3: 2.488); mean $\pm$ sd over 3 seeds. ``Average'' is the mean of the four $L_{\text{after}}$ values. $\Delta\%_{\text{adj}}=100\,(L_{\text{after}}-L_{\text{before}})/(L_{\text{before}}+k)$ with
  $k=3.548$ (mean of all $L_{\text{before}}$ of this model). Bold: lowest among comparable models. $^\dagger$: $L_{\text{before}}$ clearly worse than AdamW's (perplexity $>3\%$ higher), so these rows are not comparable.}
  \label{tab:forgetting-pythia70m}
  \fitwidth{\pgfplotstabletypeset[col sep=comma, string type, every head row/.style={before row=\toprule, after row=\midrule},
    every last row/.style={after row=\bottomrule},
    columns={optimizer,before,codeparrot,stackmathqa,musicpile,tulu3,avg,smooth},
    columns/optimizer/.style={column name=Optimizer, string type, column type=l},
    columns/before/.style={column name={$L_{\text{before}}$}, string type, column type=c},
    columns/codeparrot/.style={column name={$L_{\text{after}}$ codeparrot}, string type, column type=c},
    columns/stackmathqa/.style={column name={$L_{\text{after}}$ stackmathqa}, string type, column type=c},
    columns/musicpile/.style={column name={$L_{\text{after}}$ musicpile}, string type, column type=c},
    columns/tulu3/.style={column name={$L_{\text{after}}$ tulu3}, string type, column type=c},
    columns/avg/.style={column name={$L_{\text{after}}$ average}, string type, column type=c},
    columns/smooth/.style={column name={$\Delta\%_{\text{adj}}$}, string type, column type=c}]{\curveroot/data/forgetting_table_pythia70m.csv}}
\end{table*}


==> paper_figures_v2_old/common/preamble.tex <==
% AUTO-GENERATED by tools/make_forgetting_figures.py
\usepackage{booktabs,pgfplots,pgfplotstable,xcolor}
\usepgfplotslibrary{statistics}
\pgfplotsset{compat=1.17}
\providecommand{\figroot}{paper_figures_v2}  % folder that contains data/

\definecolor{c-codeparrot}{HTML}{0072B2}
\definecolor{c-stackmathqa}{HTML}{E69F00}
\definecolor{c-musicpile}{HTML}{009E73}
\definecolor{c-tulu3}{HTML}{CC79A7}

\pgfplotsset{
  dpt bars/.style={ybar, width=\textwidth, height=0.30\textwidth, bar width=2.6pt, ymin=0, enlarge x limits=0.045,
    ymajorgrids, grid style={gray!25}, xtick=data, x tick label style={rotate=35, anchor=east, font=\scriptsize},
    tick label style={font=\scriptsize}, label style={font=\footnotesize}, title style={font=\footnotesize},
    xlabel={Pretraining optimizer}, ylabel={Forgetting $\Delta$PT (FineWeb loss rise)}, scaled y ticks=false,
    legend style={font=\scriptsize, at={(0.5,1.02)}, anchor=south, legend columns=5, draw=none},
    error bars/y dir=both, error bars/y explicit, error bars/error bar style={line width=0.4pt}},
}


==> paper_figures_v2_old/figure_forgetting.tex <==
% AUTO-GENERATED: one full-width figure per model (needs common/preamble.tex in the preamble)
\begin{figure*}[t]
  \centering
  \resizebox{\ifdim\width>\textwidth\textwidth\else\width\fi}{!}{\input{\curveroot/forgetting_nanogpt.tex}}
  \caption{Catastrophic forgetting of nanoGPT (GPT-2 small) models pretrained with each optimizer, after fine-tuning on four datasets. Bars: rise $\Delta$PT of the held-out FineWeb-Edu loss at a common fine-tuning loss (lower is better); diamond: average over datasets; error bars: standard deviation over 3 pretraining seeds. $^\dagger$ starting model clearly weaker than \adamw's (not comparable).}
  \label{fig:forgetting-nanogpt}
\end{figure*}

\begin{figure*}[t]
  \centering
  \resizebox{\ifdim\width>\textwidth\textwidth\else\width\fi}{!}{\input{\curveroot/forgetting_pythia70m.tex}}
  \caption{Catastrophic forgetting of Pythia-70M models pretrained with each optimizer, after fine-tuning on four datasets. Bars: rise $\Delta$PT of the held-out FineWeb-Edu loss at a common fine-tuning loss (lower is better); diamond: average over datasets; error bars: standard deviation over 3 pretraining seeds. $^\dagger$ starting model clearly weaker than \adamw's (not comparable).}
  \label{fig:forgetting-pythia70m}
\end{figure*}


==> paper_figures_v2_old/forgetting_nanogpt.tex <==
% AUTO-GENERATED: grouped bars = forgetting per fine-tuning dataset, diamond = average over datasets; error bars = sd over 3 seeds
% needs \usepackage{pgfplots,pgfplotstable}; the table is loaded here (comma separated) so that optimizer names can be used as x tick labels
\definecolor{fg-codeparrot}{HTML}{0072B2}
\definecolor{fg-stackmathqa}{HTML}{E69F00}
\definecolor{fg-musicpile}{HTML}{009E73}
\definecolor{fg-tulu3}{HTML}{CC79A7}
\pgfplotstableread[col sep=comma]{\curveroot/data/forgetting_nanogpt.csv}\forgetTabNanoGPT
\begin{tikzpicture}
\begin{axis}[
  ybar, width=0.9\textwidth, height=0.30\textwidth, bar width=2.6pt, ymin=0, enlarge x limits=0.045,
  ymajorgrids, grid style={gray!25}, xtick=data, xticklabels from table={\forgetTabNanoGPT}{label},
  x tick label style={rotate=35, anchor=east, font=\scriptsize}, tick label style={font=\scriptsize}, label style={font=\footnotesize},
  title={nanoGPT (GPT-2 small)}, title style={font=\footnotesize, yshift=0.55cm}, xlabel={Pretraining optimizer},
  ylabel={Forgetting $\Delta$PT (FineWeb loss rise)}, scaled y ticks=false,
  legend style={font=\scriptsize, at={(0.5,1.02)}, anchor=south, legend columns=5, draw=none},
  error bars/y dir=both, error bars/y explicit, error bars/error bar style={line width=0.4pt}]
\addplot[bar width=2.6pt, bar shift=-3.9pt, fill=fg-codeparrot, draw=none, mark=none] table[col sep=comma, x=idx, y=codeparrot, y error=codeparrot_sd]{\curveroot/data/forgetting_nanogpt.csv};
\addlegendentry{codeparrot}
\addplot[bar width=2.6pt, bar shift=-1.3pt, fill=fg-stackmathqa, draw=none, mark=none] table[col sep=comma, x=idx, y=stackmathqa, y error=stackmathqa_sd]{\curveroot/data/forgetting_nanogpt.csv};
\addlegendentry{stackmathqa}
\addplot[bar width=2.6pt, bar shift=1.3pt, fill=fg-musicpile, draw=none, mark=none] table[col sep=comma, x=idx, y=musicpile, y error=musicpile_sd]{\curveroot/data/forgetting_nanogpt.csv};
\addlegendentry{musicpile}
\addplot[bar width=2.6pt, bar shift=3.9pt, fill=fg-tulu3, draw=none, mark=none] table[col sep=comma, x=idx, y=tulu3, y error=tulu3_sd]{\curveroot/data/forgetting_nanogpt.csv};
\addlegendentry{tulu3}
\addplot[only marks, bar shift=0pt, mark=diamond*, mark size=2.6pt, color=black, fill=black] table[col sep=comma, x=idx, y=avg, y error=avg_sd]{\curveroot/data/forgetting_nanogpt.csv};
\addlegendentry{average}
\end{axis}
\end{tikzpicture}


==> paper_figures_v2_old/forgetting_pythia70m.tex <==
% AUTO-GENERATED: grouped bars = forgetting per fine-tuning dataset, diamond = average over datasets; error bars = sd over 3 seeds
% needs \usepackage{pgfplots,pgfplotstable}; the table is loaded here (comma separated) so that optimizer names can be used as x tick labels
\definecolor{fg-codeparrot}{HTML}{0072B2}
\definecolor{fg-stackmathqa}{HTML}{E69F00}
\definecolor{fg-musicpile}{HTML}{009E73}
\definecolor{fg-tulu3}{HTML}{CC79A7}
\pgfplotstableread[col sep=comma]{\curveroot/data/forgetting_pythia70m.csv}\forgetTabPythia
\begin{tikzpicture}
\begin{axis}[
  ybar, width=0.9\textwidth, height=0.30\textwidth, bar width=2.6pt, ymin=0, enlarge x limits=0.045,
  ymajorgrids, grid style={gray!25}, xtick=data, xticklabels from table={\forgetTabPythia}{label},
  x tick label style={rotate=35, anchor=east, font=\scriptsize}, tick label style={font=\scriptsize}, label style={font=\footnotesize},
  title={Pythia-70M}, title style={font=\footnotesize, yshift=0.55cm}, xlabel={Pretraining optimizer},
  ylabel={Forgetting $\Delta$PT (FineWeb loss rise)}, scaled y ticks=false,
  legend style={font=\scriptsize, at={(0.5,1.02)}, anchor=south, legend columns=5, draw=none},
  error bars/y dir=both, error bars/y explicit, error bars/error bar style={line width=0.4pt}]
\addplot[bar width=2.6pt, bar shift=-3.9pt, fill=fg-codeparrot, draw=none, mark=none] table[col sep=comma, x=idx, y=codeparrot, y error=codeparrot_sd]{\curveroot/data/forgetting_pythia70m.csv};
\addlegendentry{codeparrot}
\addplot[bar width=2.6pt, bar shift=-1.3pt, fill=fg-stackmathqa, draw=none, mark=none] table[col sep=comma, x=idx, y=stackmathqa, y error=stackmathqa_sd]{\curveroot/data/forgetting_pythia70m.csv};
\addlegendentry{stackmathqa}
\addplot[bar width=2.6pt, bar shift=1.3pt, fill=fg-musicpile, draw=none, mark=none] table[col sep=comma, x=idx, y=musicpile, y error=musicpile_sd]{\curveroot/data/forgetting_pythia70m.csv};
\addlegendentry{musicpile}
\addplot[bar width=2.6pt, bar shift=3.9pt, fill=fg-tulu3, draw=none, mark=none] table[col sep=comma, x=idx, y=tulu3, y error=tulu3_sd]{\curveroot/data/forgetting_pythia70m.csv};
\addlegendentry{tulu3}
\addplot[only marks, bar shift=0pt, mark=diamond*, mark size=2.6pt, color=black, fill=black] table[col sep=comma, x=idx, y=avg, y error=avg_sd]{\curveroot/data/forgetting_pythia70m.csv};
\addlegendentry{average}
\end{axis}
\end{tikzpicture}


==> paper_figures_v2_old/table_forgetting.tex <==
% AUTO-GENERATED: full-width table, numbers read from data/forgetting_table.csv
\begin{table*}[t]
  \centering
  \small
  \caption{Held-out FineWeb-Edu loss $L$ of models pretrained with each optimizer, before ($L_{\text{before}}$) and after ($L_{\text{after}}$) fine-tuning
  on a new dataset (lower is better; forgetting $\Delta\mathrm{PT}=L_{\text{after}}-L_{\text{before}}$). $L_{\text{after}}$ is averaged over four fine-tuning
  datasets, each at a common fine-tuning loss; mean $\pm$ sd over 3 seeds. Bold: lowest $L_{\text{after}}$ among comparable models.
  $^\dagger$: $L_{\text{before}}$ clearly worse than \adamw's (perplexity $>3\%$ higher), so these rows are not comparable.}
  \label{tab:forgetting}
  \pgfplotstabletypeset[col sep=comma, string type, every head row/.style={before row=\toprule, after row=\midrule},
    every last row/.style={after row=\bottomrule},
    columns={optimizer,nano_before,nano_after,pythia_before,pythia_after},
    columns/optimizer/.style={column name=Optimizer, string type, column type=l},
    columns/nano_before/.style={column name={nanoGPT $L_{\text{before}}$}, string type, column type=c},
    columns/nano_after/.style={column name={nanoGPT $L_{\text{after}}$}, string type, column type=c},
    columns/pythia_before/.style={column name={Pythia-70M $L_{\text{before}}$}, string type, column type=c},
    columns/pythia_after/.style={column name={Pythia-70M $L_{\text{after}}$}, string type, column type=c}]{\figroot/data/forgetting_table.csv}
\end{table*}


==> sections/SOMA_forgetting_exp_extra.tex <==
\section{Fine-tuning curves}
Figure~\ref{fig:trainloss}  show how each pretrained model learns the four new datasets in the forgetting experiment. Every model is
fine-tuned with the same recipe,
so differences between curves come from the optimizer used for pretraining. Rows are
nanoGPT and Pythia-70M, columns are the fine-tuning datasets, and each curve is the mean
over three seeds.
\input{SOMA_exp2/figure_train_loss}

==> sections/optim_train_loss.tex <==
% \subsection{Fine-tuning training loss: nanoGPT}
\input{SOMA_exp/SOMA_exp2/figure_train_loss}


